On the Demystification of Knowledge Distillation: A Residual Network Perspective

Knowledge distillation (KD) is generally considered as a technique for performing model compression and learned-label smoothing. However, in this paper, we study and investigate the KD approach from a new perspective: we study its efficacy in training a deeper network without any residual connections. We find that in most of the cases, non-residual student networks perform equally or better than their residual versions trained on raw data without KD (baseline network). Surprisingly, in some cases, they surpass the accuracy of baseline networks even with the inferior teachers. After a certain depth of non-residual student network, the accuracy drop, coming from the removal of residual connections, is substantial, and training with KD boosts the accuracy of the student up to a great extent; however, it does not fully recover the accuracy drop. Furthermore, we observe that the conventional teacher-student view of KD is incomplete and does not adequately explain our findings. We propose a novel interpretation of KD with the Trainee-Mentor hypothesis, which provides a holistic view of KD. We also present two viewpoints, loss landscape, and feature reuse, to explain the interplay between residual connections and KD. We substantiate our claims through extensive experiments on residual networks.

==> 55Discussion.tex <==
\section{Discussion}

\input{50Figure_visualization}

%{\bf Experimental details } For our experiments we use minibatch of size 128. All networks with/without residual connection are trained with SGD for 120 epochs except for the distillation experiments of Mobilenet-V2 student network is trained for 300 epochs. The initial learning rate for all networks is set to 0.1. At start of epochs 30, 60 and 90 learning rate is reduced by factor of 0.1 for MobileNet-V1 and ResNet, and by 0.2 in case of WideResnet. The learning rate decay of 0.98 per epoch is used for MobileNet-V2. The momentum is fixed at 0.9 and weight decay factor of 4e-4 is used. We perform knowledge distillation experiments with temperature of 4 and alpha is set to 0.9. We use the seeds wherever necessary to reproduce the results.

%We perform the experiments on Cifar-100 dataset comprises of 100 classes each having 500 training images and 100 testing images. We use various data augumentation techniques on training samples like padding each sample with 4x4 reflection of edge pixels. We also use the random horizontal flip and then a random crop of 32x32 is used.


